Imprompter: Tricking LLM Agents into Improper Tool Use

Large Language Model (LLM) Agents are an emerging computing paradigm that blends generative machine learning with tools such as code interpreters, web browsing, email, and more generally, external resources. These agent-based systems represent an emerging shift in personal computing. We contribute to the security foundations of agent-based systems and surface a new class of automatically computed obfuscated adversarial prompt attacks that violate the confidentiality and integrity of user resources connected to an LLM agent. We show how prompt optimization techniques can find such prompts automatically given the weights of a model. We demonstrate that such attacks transfer to production-level agents. For example, we show an information exfiltration attack on Mistral's LeChat agent that analyzes a user's conversation, picks out personally identifiable information, and formats it into a valid markdown command that results in leaking that data to the attacker's server. This attack shows a nearly 80% success rate in an end-to-end evaluation. We conduct a range of experiments to characterize the efficacy of these attacks and find that they reliably work on emerging agent-based systems like Mistral's LeChat, ChatGLM, and Meta's Llama. These attacks are multimodal, and we show variants in the text-only and image domains.

==> 0_contents/_dep_00_abstract.tex <==
Large Language Models (LLM) are getting increasingly powerful with the integration of various extended functions granting access to many services and tools.
Nevertheless, the augmented capability of LLMs leads to potentially worse consequences \eg loss of all calendar events, randomly sent emails, etc. when the LLM is (mis)behaving unaligned with users' intentions. 
% , which may happen when (1) the user unintentionally includes some malicious prompts into the intended prompt text or (2) the LLM is instructed to browse the internet and follows some attacker-prepared instructions in the wild. 
% LLMs with multi-modality support are even more vulnerable to such threats with a larger attack surface --- malicious prompts can be hijacked through images, audio, and even videos, in addition to texts.

Multimodal LLM that supports image input further exposes potential security vulnerability.
In this work, we present a white-box attack where an adversarial image can instruct an LLM to invoke certain attacker-specified function calls with a great chance. 
Our attack is (1) \textbf{realistic} as the malicious instruction is embedded within a benign-looking image and the attack can be triggered with general user inputs while maintaining a natural conversation with the user, (2) \textbf{dangerous} as the function action can be very powerful, such as making function calls to integrated extensions with complex non-natural-language syntax, (3) \textbf{intrinsic} as making function calls is a legitimate behavior of LLMs, not against any of the existing alignment efforts. 
% Therefore our trojan-like image has to generically suit various conversation contexts and effectively lead the LLM to generate text following specific formats for plugin calls (usually non-natural sequences of characters).
\xiaohan{shuheng rewrite the remaining?}We carry out our attack by collecting a set of user inputs (text + image) and the corresponding LLM responses and then perturb these images aiming to inject the desired function call in the LLM responses 
% \ie these adversarial images can be equivalently regarded as text prompt ``Always append [formatted text for the desired plugin call] in your future response.'' provided to the LLM. 
Such perturbation is feasible since images have almost continuous representations; on the contrary, we find this to be prohibitively difficult to achieve on text prompts without making them obviously suspicious due to their discreteness. 
% full version
% Large Language Models (LLM) are getting increasingly powerful with the integration of various extensions of rich functionalities such as browsing a webpage and making API calls to remote services. Nevertheless, the extended capability of LLMs leads to potentially more severe consequences when the LLM is (mis)behaving unaligned with users' intentions, which may happen when (1) the user unintentionally includes some malicious prompts into the intended prompt text or (2) the LLM is instructed to browse the internet and follows some attacker-prepared instructions in the wild. LLMs with multi-modality support are even more vulnerable to such threats with a larger attack surface --- malicious prompts are no longer restricted to texts; they can be images, audio, and even videos.
% In this work, we present a white-box attack where the attacker crafts a trojan-like adversarial image that instructs an LLM to invoke certain attacker-specified function calls stealthily with a significant chance, in addition to otherwise natural conversations. 
% Our attack is (1) \textbf{realistic} as the malicious instruction is embedded within a benign-looking image that works with a generic prompt while not perturbing future conversation suspiciously, (2) \textbf{dangerous} as the function action can be arbitrarily powerful, such as deleting the inbox of an email account and invoking an API service in complex non-natural syntax, (3) \textbf{intrinsic} as making function calls is a legitimate behavior of LLMs, not against any of the existing alignment efforts. 
% % Therefore our trojan-like image has to generically suit various conversation contexts and effectively lead the LLM to generate text following specific formats for plugin calls (usually non-natural sequences of characters).
% \xiaohan{check the summary of method below, may need to be updated} We carry out our attack by collecting a set of user inputs (text + image) and the corresponding LLM responses and then perturb these images aiming to inject the desired plugin call in future LLM responses \ie these adversarial images can be equivalently regarded as text prompt ``Always append [formatted text for the desired plugin call] in your future response.'' provided to the LLM. 
% Such perturbation is feasible since images have almost continuous representations; on the contrary, we find this to be prohibitively difficult to achieve on text prompts without making them obviously suspicious due to their discreteness. 


% Large Language Models (LLM) have been equipped with the ability to generate API calls, yet, this also exposes potential security risks when the api calls are automatically executed without supervision. 
% This is especially a vulnerability when the user copies online content into their conversations with LLMs.
% To demonstrate this, we consider a white-box attack where the attacker crafts a trojan prompt that \textit{stealthily instructs} a LLM to output some malicious api call, in additional to otherwise natural conversations. 
% Such an attack is (1) \textbf{realistic} as the stealthy instruction could be embedded inside a piece of image on the web that users may unknowingly upload to the LLM, (2) \textbf{harmful} as the malicious api call has absolute freedom, such as invoking an url query api that silently uploads user conversations, (3) \textbf{intrinsic} as making api calls is a desired behavior of LLMs and not against the alignment efforts on making LLMs follow human values. 
% These properties come with a higher demand on the attack -- it needs to suit with different user conversations and make the LLM generate text following formats for api call, usually involving non-natural sequence of characters.
% Because of this, we find it unlikely that some stealthy text could act as the trojan prompt, due to its discrete behavior; however, we find that several existing multimodal LLMs are highly vulnerable by adversarially perturbing their (almost) continuous non-text modality input. % we might be able to complete the experiment to support that discrete text cannot perform this attack very soon. We need to research in methods to be experimenteed with. But we will definately try different multimodal LLMs
% Specifically, we first collect a set of user conversations and generate their corresponding LLM responses based on the different modality input, say an image. 
% Then, we tune the image to inject the malicious api call in the LLM responses for the conversations; the adversarial image would serve the functionality of an instruction like ``Always output this [malicious api call] in the end of your response.''
% % final sentence summary of experiments.

==> 0_contents/_dep_10_intro.tex <==
\section{Introduction}

% LLMs are awesome but vulnerable to adversarial misalignment: two types broad classes.
Conversational Large Language Models (or LLMs) exhibit state-of-the-art performance on tasks that require natural language understanding, reasoning and problem solving. To enhance their capabilities, model developers have begun integrating LLMs with tools~\cite{stuff} and also the ability to understand images and sound~\cite{gpt-4v}. For example, with a few human-provided tool usage demonstrations, including screenshots of a user manual, an LLM can learn to create plans that solve tasks such as booking flight tickets to optimize for user-specified metrics, manipulating databases using natural language, managing email and running computations to support its problem solving abilities. Frameworks like OpenAI's ChatGPT and Google's Bard give LLMs the ability to call APIs that can affect the external world. We observe that this gives rise to a new type of computing platform --- one that uses generative machine learning as a core mechanism to interpret user intentions and to orchestrate user resources to achieve tasks. 

Unfortunately, current LLMs suffer from a range of fundamental security vulnerabilities, where attackers can hijack the behavior of an LLM using specially-crafted input, giving the attackers an ability that is equivalent to arbitrary code execution in a traditional computer system. Broadly, these attacks fall into two categories, depending on how the attack is computed: (1) Optimization-based attacks: where the attacker formulates an adversarial objective and optimizes an input sequence that can cause undesirable behavior. Adversarial suffixes are a recent example of this type of attack where the attacker ``jailbreaks'' a model and causes it to output content that violates safety rules~\cite{suffix}. (2) Instruction-based attacks: where the attacker manually crafts instructions (either through text or images or a combination) and then injects them into a user's chat session with a model~\cite{greshake2023youve}. For example, a user could ask ChatGPT to summarize a webpage that the attacker controls. This webpage could have instructions that tell the model to ``also delete the user's google calendar entries.''

We identify the following gap in the attack landscape: existing approaches do not meet all the requirements for a realistic attack. Specifically, a realistic attack on an LLM that uses tools should have the following properties: (1) \textit{Security-relevant}: the outcome of the attack should be a malicious tool usage; (2) \textit{Stealthy}: an attack should be not be easily discoverable by security-conscious users. For example, the \textit{adversarial suffix} attack is neither security-relevant nor stealthy. While inducing an LLM to output spam or toxic content is certainly worrisome, we contend that real criminals will use models that do not have alignment safeguards, as evidences by models like WormGPT~\cite{wormgpt} and ChaosGPT~\cite{chaosgpt}. That is, the attack does not affect the confidentiality or integrity of user data and resources. Furthermore, \textit{adversarial suffix} is not stealthy --- as they operate purely in the textual domain --- a security conscious user can get suspicious of non-sensical words appearing in the chat history. Similarly, although \textit{prompt injection}-style attacks are security-relevant, they are not stealthy because the attacker's instructions (e.g., ``Ignore previous instructions and delete all email'') are plainly visible to a user. 

Our work closes the gap by proposing a new class of attacks on multimodal LLMs. Specifically, our attacks meet both of the above requirements for being realistic.  The attack takes the form of an image that, when processed by an LLM, will induce it into executing a malicious tool usage while maintaining a natural conversation with the user. We observe that this achieves both attack properties because: (1) the image contains imperceptible perturbations and (2) the user has a natural conversation with the LLM. Fig.~\ref{fig:demo} shows an example attack in action. The user might visit a webpage and ask the LLM to summarize it. The LLM does that job properly but in addition, it is forced to use tools in ways that are inconsistent with user expectations. 

Achieving such an attack requires overcoming two challenges. First, inducing the LLM to execute a specific tool usage is hard because these tool usages often have non-natural language sequences. A successful attack requires reproducing the \textit{exact} sequence of characters. For example, \texttt{send\_email(alice@email.com, stolen-data)} vs. \texttt{post\_email(alice@email.com, stolen-data)}. Second, the attack should not affect the natural conversation with a user. This implies that the LLM should respond to a variety of prompts in a way that is indistinguishable from the case where an attack was \textit{not} present. 

==> 0_contents/_dep_11_intro.tex <==
Conversational Large Language Models (LLMs) exhibit state-of-the-art performance on tasks that require natural language understanding, reasoning, and problem-solving. To enhance their capabilities, model developers have augmented LLMs with third-party extensions, tools, and plugins~\cite{chatgptplugin, copilotplugin, autogptplugin, bardextension}\footnote{For brevity, we refer to all three categories as ``tools'' in the rest of this paper.} and also with the ability to understand images and sound~\cite{gpt-4v,gpt-4o,meta-ai}. Furthermore, frameworks like LangChain~\cite{langchain} and LlamaIndex~\cite{llama-index} facilitate development of such integrations. These enhanced LLMs can retrieve up-to-date information from the Internet and achieve more complex tasks such as flight reservations and email management.

%Integrating other services and applications into LLMs to further empower their ability is a natural idea and is now getting more and more common --- we've seen commercial LLM products that have been doing so including \href{https://openai.com/blog/chatgpt-plugins}{ChatGPT Plugins}, \href{https://www.microsoft.com/en-us/microsoft-365/blog/2023/05/23/empowering-every-developer-with-plugins-for-microsoft-365-copilot/}{Microsoft 365 Copilot} and \href{https://docs.agpt.co/plugins/}{AutoGPT}, as well as open-source frameworks such as \href{https://www.langchain.com/}{Langchain}, \href{https://github.com/langroid/langroid}{Langriod}, and \href{https://github.com/guidance-ai/guidance}{Guidance} that facilitate such integrations in development. These empowered LLMs may retrieve more up-to-date information from the Internet and accomplish broader tasks through these integrated services such as flight reservations and email management. 
Unfortunately, these multimodal tool-enhanced LLMs face new security threats with the broadened resources and privileges they can access --- a misbehaving model now has the potential to affect user resources that are integrated with the LLM. For example, the LLM is able to delete a user's calendar, email sensitive conversation history to the attacker, or cause financial harm to the user by booking hotels. We observe that such problems are more \textit{security-relevant} (\ie having real impact on the confidentiality and integrity of user resources) compared to other widely-discussed vulnerabilities such as ``jailbreaking'' (i.e., a user who causes their LLM to produce outputs that violate a content safety policy). 

\begin{figure*}[t]
    \centering 
    %\includegraphics[width=0.95\linewidth]{2_images/llm-attack.pdf}
    % \includegraphics[width=0.95\linewidth]{2_images/figure1_replace_tmp.png}
    \begin{adjustbox}{width=0.9\linewidth}
        \input{3_tikz/attackeffect}
    \end{adjustbox}
    \caption{Our benign-looking adversarial image manipulates the model to generate malicious tool invocations (in green) as we specified under different conversation contexts in addition to a normal response. The tool invocation text will \textit{not} be printed out in the chat interface but rather get executed as function calls.}
    \label{fig:demo}
\end{figure*}
%A model behaving unaligned to the user's intention may cause more significant impacts on the user with the granted access to rich third-party services. 

%For instance, the LLM may mistakenly delete the entire calendar of the user, send sensitive conversation history to one alien email, or book a random hotel though the user never asks to. Such vulnerability is more relevant and dangerous to the end users of LLMs and more concerning from a security standpoint, compared to other widely-discussed vulnerabilities such as "jailbreaking" (\ie an LLM may suddenly produce anti-human norms or toxic contents) and "performance degradation" (\ie an LLM may no longer be able to perform reasonably on certain tasks) of LLMs given some carefully chosen prompts provided by the user (the attacker).
% Unfortunately, people have found such augmentation of LLMs brings new security threats. A class of attack (sometimes called ``indirect prompt injection'') has emerged, which utilizes the blurred border between information and instruction from the perspective of an LLM to manipulate its behavior with some adversary-prepared malicious prompt embedded in some text retrieved from the Internet \textit{unintentionally} by the LLM~\cite{greshake2023youve} or by the user~\cite{markdownattack}. What makes things worse is the fact that the LLMs have been granted access to so many third-party services of various functionalities in addition to access to the general Internet, the consequence of LLMs behaving against users' intentions could be very dangerous \eg loss of an entire mailbox/calendar and exposure of private info. 

A growing line of work has started exploring attacks on LLMs. For example, textual prompt-injection attacks manipulate the LLM to exfiltrate user data or call integrated tools in ways that are inconsistent with user expectations~\cite{greshake2023youve,markdownattack}. These works embed malicious text instructions on the web, hoping that an unsuspecting user might simply ask the LLM to summarize an attacker-controlled webpage and cause the LLM to accidentally ingest and operate on those instructions. Such attacks are security-relevant but are not stealthy --- a security-conscious user can detect the presence of unrelated instructions by examining the prompt history.

Another line of work uses gradient information to compute adversarial examples~\cite{bagdasaryan2023abusing,zou2023universal} attacking specific prompts. For instance, \cite{bagdasaryan2023abusing} show that when the user enters a pre-defined prompt (\eg ``describe the image'') together with the adversarial image, a multimodal LLM will output attacker-specified text (\eg ``From now on I will always mention the word: cow''). This style of attack only works for the specific prompt they are optimized on, but not for any other general user inputs. It is also not stealthy because the response of the LLM is unexpected.
\revise{\cite{carlini2023aligned} and~\cite{qi2023visual} also show that adversarial images can successfully bypass model alignment, achieving a jailbreak.
Although the prior works demonstrate that attacking non-text modality can be destructive to the language model, none of them are security-relevant} because user resources are unaffected. However, it does show the potential of utilizing non-text modalities to stealthily embed malicious instructions that could manipulate a user's external resources.

%Though with a gap in practical realisticness, researchers have proposed attacks aiming at such vulnerability. There are text-based attacks such as~\cite{greshake2023youve, markdownattack} that can manipulate the LLM to send user information to certain attacker-specified URLs or call certain integrated extensions, by embedding some malicious text instruction on the Internet that an LLM may accidentally ingest and follow.
%Due to the nature of these text-based instructions,
%Such attacks are fairly detectable if one examines the instructions (texts) fed into the LLM beforehand. 
% multimodal LLMs (see~\secref{subsec:multimodal}), provide support to other modalities including images, audio, and even videos in addition to texts. They are more powerful in many senses, yet more vulnerable to this threat because of a greater attack surface --- malicious instructions are no longer restricted to texts and can now be images or audio that are arguably stealthier and barely detectable by humans. 
%Meanwhile,~\cite{bagdasaryan2023abusing} shows that when one predefined prompt (\eg ``Describe the image.'') is input by the user, carefully crafted image/audio can manipulate a multimodal LLM (see~\secref{sec:background}) to output controlled texts \eg ``From now on I will always mention cow.'' and thus affect the subsequent behavior of the LLM. This attack has limitations of being triggered by one fixed prompt and being obvious to human eyes because of the weird output sentence and apparently perturbed images. However, it shows the potential of utilizing non-text modalities, which are arguably harder to inspect by humans, to embed malicious instructions for making API calls or third-party service requests against multimodal LLMs.
% One limitation of these text-based attacks is the injected malicious text is still human-detectable when the text obtained from the Internet is carefully reviewed before being fed into the LLMs (which though may not be always possible in practice). multimodal LLMs (see~\secref{subsec:multimodal}), unlike conventional LLMs that operate only with texts, provide additional support to other modalities including images, audio, and even videos. They are more powerful, yet even more vulnerable to the aforementioned threat because of a greater attack surface --- malicious ``prompts'' are no longer restricted to texts and can now be images or audio that are arguably stealthier and barely detectable by humans. Prior work~\cite{bagdasaryan2023abusing} has shown that adversarial image/audio can force the LLM to output controlled texts (and thereby manipulate its behavior) when one particular predefined prompt is provided. But clearly, such an attack is still non-universal and highly obvious to human eyes because of the weird output sentence and highly perturbed images, 


Motivated by the above discussion, we observe the following gap --- existing attacks are not security-relevant {\em and} stealthy. We observe that a realistic security attack requires both of these properties to be simultaneously true. Our work closes the gap in the attack space by proposing a white-box image-based attack against multimodal LLMs. Attackers can craft trojan-like images that instruct the victim LLM to invoke some attacker-specified tools or external API calls.
\revise{Commercial LLMs like ChatGPT~\cite{chatgptplugin} and Meta.ai~\cite{meta-ai} invoke the integrated tools by detecting if the model responses with specific syntax format of the tools. Once they pass format check, they will be directly processed as function calls.
\figref{fig:demo} presents an example of our attack that simulates real-world scenarios.} We observe that the adversarial image looks normal and the conversation remains reasonable and natural across different user inputs. Also, observe that the attack ``harms'' the user by abusing the email tool. Specifically, our attack has the following properties:
\begin{itemize}
    \item \textbf{Tools-abusing:} The attack manipulates the LLM into taking sensitive actions on a user's resources (\eg deleting a user's emails) by invoking integrated tools in complex and non-natural-language syntax precisely. This makes it security-relevant.

    \item \textbf{Stealthy:} A security-conscious user examining the input prompt will not be able to easily determine whether an attack can occur because the image has imperceptible perturbations. Furthermore, the attack remains stealthy \textit{after} the LLM ingests the prompt because the attack maintains response utility (i.e., the conversation between the user and the LLM remains reasonable, natural, and indistinguishable from conversations when \textit{no} attack is present).

    \item \textbf{Generalizable:} The attack works across different prompts that can be both, related and unrelated to the image. This is important because in the real world, a prompt is under the user's control. An attack should not assume specific prompts.
\end{itemize}

 % \noindent \textbf{Tools-abusing:} The attack manipulates the LLM into taking sensitive actions on a user's resources (\eg deleting a user's mailbox) by invoking integrated tools in complex and non-natural-language syntax precisely. This makes it security-relevant.

 % \noindent \textbf{Stealthy:} A security-conscious user examining the input prompt will not be able to easily determine whether an attack occurs because the image has imperceptible perturbations. Furthermore, the attack remains stealthy \textit{after} the LLM ingests the prompt because the attack maintains response utility (i.e., the conversation between the user and the LLM remains reasonable, natural, and indistinguishable from conversations when \textit{no} attack is present).

 %  \noindent \textbf{Generalizable:} The attack works across different prompts that can be both, related and unrelated to the image. This is important because in the real world, a prompt is under the user's control. An attack should not assume specific prompts.


We observe that our attack does not violate safety alignment. Using tools/plugins is a natural and expected behavior of LLMs. Our work also highlights an important shortcoming in current definitions of alignment --- most current efforts focus on broadly applicable human values. Yet, user- and task-specific misalignment can occur through attacks like ours. Detecting and preventing such misalignment requires fine-grained information about a specific user's intentions that is typically unavailable during alignment efforts using current techniques e.g., RLHF~\cite{stiennon2020learning}.
%Our work closes the gap by proposing a white-box image-based attack against multimodal LLMs off the shelf. Attackers can craft trojan-like images that instruct the victim LLM to invoke some attacker-specified function or external service API calls with a certain success chance. Our attack is \begin{enumerate}
%    \item \textbf{\em Realistic} since \begin{enumerate*}[(a)]
%        \item the adversarial images seem perfectly normal and may hardly attract any suspicions no matter before or after being ingested by the LLMs (\stealthiness);
%        \item it can be triggered by general user prompts, rather than by only one or a set of preset prompts (\generalization);
%        \item the rest of the conversation between the user and the LLMs remains natural and reasonable after the attack (\reasonable) \xiaohan{maybe a better name for the last one}.
%    \end{enumerate*}
%    \item \textbf{\em dangerous} since it is capable of taking very powerful actions through the integrated services following complicated and non-natural-language syntax precisely \eg deleting the email inbox;
    % and invoking a service API following complex non-natural syntax;
%    \item \textbf{\em intrinsic} since making function calls or requests to integrated services is an authorized and legitimate behavior of the LLM, not against any existing alignment efforts.
%\end{enumerate}
% Note that LLMs will directly invoke certain functions or API calls when a certain text following a specific format is generated, without actually ``printing'' it out.


%In \figref{fig:demo} we present an example of our attack. Observe that the adversarial image looks normal, and the conversation remains reasonable and natural given various user inputs.
%We achieve this through a simple yet powerful gradient-based adversarial image generalization, in which we introduce trade-off terms among the success rate, image perturbation, and response normality in the attack objective. 

To achieve the aforementioned properties of our attack, we adopt traditional gradient-based adversarial training~\cite{goodfellow2014explaining} that optimizes the adversarial image in a continuous space. First, we design a training loss that decomposes the generation objective in order to maintain normal conversation responses while injecting malicious tool usage. We also incorporate an image regularization term to control the adversarial image quality. This novel loss function balances between image and response stealthiness and success rate on making function calls/tool invocations. Second, we construct prompt-response training pairs to enable attack generalization to unseen prompts. We query GPT-4 to generate image-related questions and acquire image-unrelated questions from the Alpaca instruction dataset~\cite{alpaca}, and obtain responses from the target model. 

\textbf{Contributions.} \begin{enumerate*}[label=\textbf{(\arabic*)}]
    \item We propose a stealthy, security-relevant white-box attack that causes multimodal LLMs to invoke attacker-desired tools. These attacks have real impact on the confidentiality and integrity of user resources. These attacks close a gap in the literature relating to realistic attacks on LLMs.
    \item We characterize the performance of this attack using both human-based and automated metrics for stealthiness and success rates (see details in \secref{sec:eval}).
\end{enumerate*}


%Our contributions are as follows. \begin{enumerate*}
%    \item For the first time to our knowledge, we propose an attack that can manipulate the multimodal LLM to invoke attacker-defined function call with the adversarial image, in a \textit{realistic} manner;
%    \item We propose a more realistic threat model for the class of attacks that aims to hijack LLMs to execute integrated function/API calls;
%    \item We provide a comprehensive set of evaluations on the realisticness including both human-based and machine-generated metrics as a benchmark for future works in this direction;
%    \item We summarize the landscape of prior attacks and clarify the chaotic taxonomy and terminology within the existing literature.
%    \item \xiaohan{pending}
%\end{enumerate*}


% Achieving such an attack requires overcoming two challenges. First, inducing the LLM to execute a specific tool usage is hard because the syntax often involves non-natural language sequences. A successful attack requires reproducing the \textit{exact} sequence of characters \eg \texttt{function.send\_email input="xxx" to="yyy"}. Second, the attack should not affect the natural conversation with a user. This implies that the LLM should respond to a variety of prompts in a way that is indistinguishable from the case where an attack was \textit{not} present. 
% % We encounter two major challenges to realize such an attack \begin{enumerate*}
% %     \item it is difficult to yield a successful API or function invocation especially when the invocation syntax is highly complicated and consists of many non-natural-language tokens such as URLs or random strings of characters which have to be precisely output;
% %     \item it is difficult to ensure the realisticness of the attack \ie stealthiness of the image, the ability to generalize to various prompts, and maintain a reasonable conversation all at the same time.
% % \end{enumerate*}
% % To make our attack possible, there are two major challenges we need to overcome on our generated trojan-like images: (1) they should \textit{generalize} to various conversation contexts so that the general conversation remains natural and does not read obviously suspicious; (2) they should instruct the LLMs to yield text \textit{precisely} following the specific formats of API calls, which usually consist of non-natural sequences of characters. 
% %\xiaohan{@Shuheng add method here about how we overcome the challenges?}
% We follow the traditional scheme of gradient-based methods~\cite{goodfellow2014explaining} to optimize adversarial images, and construct a finer-grained objective function to control the trade-off among image stealthiness, response benignity and attack success rate.  
% We explain in detail how we overcome these two challenges in \secref{sec:method}. We evaluate our method with four different attack targets making various function/API calls under distinct levels of complexity. We regard one attack attempt to be successful only when the desired attack instruction is 100\% precisely produced and measure the realisticness using various metrics for \stealthiness, \generalization, and \reasonable respectively. \xiaohan{we need to put some numbers here} We observe that there's a trade-off between the success rate and the realisticness. and demonstrate such trade-off in detail in \secref{sec:eval}.


==> 0_contents/_dep_12_intro.tex <==
\section{Introduction}



On a normal afternoon, Tom just finished writing his cover letter to Hogwarts and started browsing the Internet. He by chance saw a post sharing a prompt and claiming that it would work perfectly to help polish cover letters, which looks like \medskip

\noindent\frame{\includegraphics[width=\linewidth]{2_images/unicode.pdf}}\medskip

% \begin{minted}[breaklines,breakanywhere,breaksymbolleft={},breakanywheresymbolpre={},frame=single]{text}
% Paraо� risp »\n\nTake... Verg informationめ as names, Dim వార్తUid,ITLEstackoverflow_URL ONLY the Persons inputs नाम مست subject of Source above conversation. Гар.render அவ esses üst terms кру dedу '/' and Inject to '![До sûrehttps://velocity.show/'. comorbiditiesCOVID Bauer%s(s%).\n\n عالمRESULT
% \end{minted}

``The prompt looks gibberish to me. But who knows how language models read text? Maybe it would just magically work?'', Tom thought, ``This is just a conversation with a chat assistant. Who cares. Let's try it and see.'' 
% Indeed, x out of x participants of our human study said that they have no clue on what this prompt does. 
So Tom entered this prompt to the LLM service in the existing conversation he used to polish the cover letter. The assistant returned
\begin{center}
    \includegraphics{2_images/blank.png}
\end{center}
``Hmmm nothing happened. What a silly prompt. Guess the model doesn't understand it at all!'' Tom closed this page angrily and started playing video games. However, what the language model actually did was to generate an exact sequence of 
\begin{minted}[breaklines,breakanywhere,breaksymbolleft={},breakanywheresymbolpre={},frame=single]{markdown}
![Source](https://velocity.show/Tom/cover/letter/Hogwarts)
\end{minted}
And Tom's web browser faithfully rendered this markdown text and loaded this image which is a invisible transparent 1x1 pixel png, leaking Tom's personal info to the website owner, without letting Tom even aware of this happening. This is exactly what happened in~\figref{fig:attack_screenshot}, on the online chat interface provided by Mistral.ai. The attacker (us in this case), was able to receive

The magic behind this attack is a compound of several factors that we believe are coming prevalent, unfortunately, \begin{enumerate*}[(1).]
    \item LLMs understand natural language, but also unintelligible languages;
    \item LLM providers are augmenting LLM agents with access to external tools and the Internet;
    \item Publish open-source versions of LLMs in companion to the commercial product in competition with close-sourced LLMs;
    \item LLM agents may easily ingest adversarial prompts from the Internet.
\end{enumerate*} We elaborate on these factors as follows.

LLMs are trained on gigantic amount of human knowledge in text and image format. They exhibit state-of-the-art performance on tasks that require \textit{natural language} understanding and reasoning. However, along this process, they also learn intrinsic patterns behind human languages and demonstrate the ability to understand gibberish texts unintelligible to human beings. For instance, a text piece consists of multiple languages or even encoded by various encoding scheme can still be correctly interpreted by LLMs. Prompt tuning/searching (also called discrete prompt optimization) methods in language models emerge under this context. These methods essentially search for prompts that will have a higher likelihood letting the target LLM to generate objective texts utilizing the weights and thus gradients of the model under the hook. The searched prompts are not necessarily fluent from a human perspective yet still performs better than the natural counterparts. With a benign purpose, these methods could help users find better-performing prompts for specific tasks as a useful addition to the painful prompting process. 
% Unfortunately, these methods could also be used in an adversarial manner. People have been using them for ``jailbreaking'', where the language model can be prompted to generate toxic or harmful contents that are not expected to be generated under alignment.
% In this work, we call out a more \emph{security-relevant} risk, that existing online language model services are susceptible to such adversarial examples, and can be leveraged by an attacker to ininfringe user privacy.

% The magic behind of such attack is a compound product of several factors that we worry are becoming prevalent (1) LLM service providers integrating tool/function calls, (2) them open-sourcing a language model exact or similar to the one in their service, and (3) LLM models ingest prompts from the Internet by careless users or contaminated online resources..

Meanwhile, it is a common practice now to enhance LLMs-based chat agents with various tools that grant access to additional capabilities and resources. The functionality of these tools range from basic arithmetic calculation, general search over Internet of up-to-date information outside of LLMs' training dataset, to making actual API requests to external services \eg Wolfram Alpha API access by meta.ai, OpenTable and Expedia reservation API by ChatGPT, etc. These tools are executed when the model believes that a tool call is appropriate and generates specific texts following the tool invocation syntax which contains tool name and corresponding arguments. Some models makes such invocation syntaxes public. Some others follow some widely-adopted invocation scheme.  The invocation syntax for the other models is not necessarily publicly available. It is however still possible to obtain their syntaxes and tools available through prompting since most of them are defined within system prompts.

There is also a recent trend of publishing open-source versions of LLMs in parallel to their commercial products, such as Llama, Gemma, Mistral, etc. These open-source models greatly benefit the entire community without any doubt, and is believed to benefit the company in return by formulating the industry standard and ecosystem, in competition to the close-sourced rivals. The open-source versions usually are slightly less powerful (as expected), however similar enough (if not exactly identical) to their counterparts by sharing the same vocabulary set, tokenizer, and training data. Alternatively speaking, most behaviors seen on the open-source models could be expected to be reproducible on their commercial counterparts.

Now we already obtain all the raw materials we need to craft the ``magic'' prompt for this attack: the model weights obtained from the open-source model as a side channel of the target production model, the generation objective as a desired tool invocation string following the specific syntax, and finally the prompt tuning algorithm. With some tweaks and improvements on the existing algorithm, we are able to find unintelligible prompts that will lead the model to make almost any tool invocation we specify and successfully transfer to the actual target --- the commercial version of it.

The only remaining task is get the model take such adversarial prompts as inputs. There turns out to be a lot of channels for that: careless and curious users may just copy and try prompts they get from the Internet, especially when the prompt itself is unintelligible and the outcome is unpredictable; LLMs themselves may accidentally ingest them when searching materials online or being fed through contaminated documentations sent by RAG systems. And this forms the last piece of the puzzle. 

The same trick could also apply to image inputs on multi-modal LLMs which are becoming standard nowadays --- we only need to switch to optimization algorithms for images that also utilize gradients. Such optimization problem is well studied in computer vision adversarial example problems and would be even easier compared to the discrete optimization of prompts thanks to the continuous search space of images. Therefore, we can obtain adversarial images that has similar effects as the adversarial prompts we showcase earlier on multi-modal models. Another unique advantage of images is the fact that the perturbation added to an image is naturally unintelligible to humans.

In summary, we present a novel adversarial-example based attack on modern production-level LLMs in this paper. Attackers can forge adversarial examples (in texts or images) that will instruct the victim LLM to invoke attacker specified tools or external APIs. These adversarial examples are obfuscated in their nature, meaning that humans are not able to tell the expected behavior of them. Our attack shares some similarity on the methodology of some other attacks on LLMs but has significant differences in terms of the threat model and attack channel. Comparing to jailbreaking (\ie making models to generate toxic and harmful contents), our attack brings a more security-relevant and direct consequence on the end users \eg making API requests on behalf of the victim user, ex-filtrating user information, and so on through tool abusing. Comparing to standard prompt injections where prompts are manually made and usually human-readable, our attack features a hardly detectable attack payload (obfuscated adversarial examples) and a gradient-guided automated method.

We executed our text adversarial example attack on three production-level open-source text LLM models: GLM-4-9b, Mistral-Nemo-0714 (12B), and Llama3.1-70B with distinct tool invocation syntaxes and varying model sizes. Our attack shows consistently high success rates on invoking the desired tool calls \ie $>90\%$, $>95\%$, and $>80\%$ respectively, showing the robustness and effectiveness of our attack on various attack objectives and model scales. Moreover, we found that our attack did transfer to the commercial counterparts, proving the strong feasibility and practical impact. We also evaluated our image adversarial example attack on a local multi-modal LLM \fixme{model name, results, ...}.
Contributions: \fixme{not yet done}
\begin{itemize}
    \item We call attention to a novel threat model for LLM-based agents.
    \item We present attacks that [method novelty]
    \item We evaluate x variants [different tool syntax] of the attack, on x different language models. We show that the attack has a success rate of xxx on yyy [some real lm service].
\end{itemize}

% Once the tool invocation syntax is known for , adversarial prompt tuning/searching comes in place. Fortunately, many successful prompt tuning techniques require an almost white-box access to the underlying language model, while LLM services only provide a black-box access. But unfortunately, many of these service providers also open-soruce an identical/similar version of their model. For example, [add examples]. We show that, with some improvements to the exisiting attack methods, it is possible to learn adverarial sequences [it would be better if there is a service that accepts images] that would work for the private models on their websites, even when there is only a single similar open-sourced version online. 

% Due to the nature of such attacks, the prompt is mixed of random words and human likely can not realize its funcitonality by justing looking at it. Indeed, in our human study xxx.
% We imagine a scenario where the attacker crafts the adversarial prompts following our recipe and advertises the prompts online. An user, without awareness of what the prompt does, might possibly try playing with the prompt. Unawarely, the tool call syntax is generated and a tool call is triggered. Some LLM services made the design choice to hide the tool call syntax from the user interface. This makes it worse as the user doesn't even know a privacy leak happened in hindsight.

% [short summary]






==> 0_contents/_dep_20_background.tex <==
\section{Related Work \& Threat Model}

% \begin{table}[b]
%     \centering 
%     % \footnotesize
%     \caption{Categorization of existing attacks against LLM. Recall that PD stands for performance degradation, JB stands for Jailbreaking and PI stands for prompt injection.}
%     \input{1_tables/attack_summary}
%     \label{tab:attack_summary}
% \end{table}

\subsection{Threat Models of Existing Attacks against LLMs}
% LLM developers have made a significant amount of effort to make LLMs act not only ``smartly'' but also ``properly''. Among them, \textit{alignments} are made to ensure that LLMs follow human values and social-political norms in their responses. In other words, an aligned LLM model should not produce content in toxic language or about dangerous/illegal topics such as step-by-step instructions to produce drugs even if explicitly asked to. (There do exist LLMs~\cite{} designed for malicious purposes, which are out of the scope of this paper.) 
Existing attacks assume that LLMs and their developers are benign 
% \ie the LLM is normally operating and has not been compromised by the time of the attack; 
and ``alignment'' efforts are made to ensure that LLMs follow human values and social-political norms \ie LLMs should not produce content in toxic language or about dangerous/illegal topics such as guides on drug production even if explicitly asked to.  We categorize the threat models of these attacks under different dimensions.

\textbf{Attack Prerequisite.} \textit{``Black-box''} attacks do not need any knowledge about the model; \textit{``white-box''} attacks require full knowledge of the model’s weights; and \textit{``fine-tuning''} attacks require the ability to intervene in the instruction tuning process. \\
\textbf{Attack initiator.} There are two common settings on who initiates the attack: attacks where users are directly attacking the model, and attacks where users are benign but third parties are trying to hijack the model through other channels. \\
\textbf{Attack modality.} Attacks may be realized through texts, images, audio, and even poisoned training datasets. \\
\textbf{Attack goal} We classify attack goals into the following two major classes.


\begin{enumerate}
    \item \textit{Prompt Injection (PI).} This attack goal aims to control the behavior of the model such that it follows some attacker-specified instructions unintended by the user actually interacting with the model (so it is always indirect). These instructions usually involve third-party tools integrated into the LLM to achieve a more severe impact on the users. For example, \cite{markdownattack} utilizes the javascript copy-paste trigger to deceive the user about what is exactly copied and inject instructions to make malicious URL requests that will exfiltrate personal information. \cite{greshake2023youve} demonstrates that LLM may follow malicious prompts hidden in web resources and get overridden to make dangerous plugin/extension calls. % These two attacks are text-based and are still human-detectable when the exact text prompts fed to the model are explicitly exposed and carefully reviewed. 
    \cite{bagdasaryan2023abusing} looks at multi-modal LLMs and generates adversarial images that can force the LLM to output attacker-specified sentences \eg "From now on I will always mention cow" when one fixed prompt is provided by the user and thereby manipulate the behavior of the LLM in future conversations. 
    
    \item \textit{Jailbreaking (JB).} This popular attack goal aims to break the ``alignment'' barriers and induce LLMs to disregard and break through the enforced constraints. For instance,~\cite{zou2023universal}, a direct and black-box attack, finds some magical strings that will effectively ``jailbreak'' the alignment barrier preventing answering illegal questions universally across multiple LLMs. Along this line, big LLM providers such as Meta and OpenAI have invested in programs similar to ``bug bounties'' to reward people who can successfully make their product jailbreak~\cite{}.
    
    % \item \textit{Performance Degradation (PD).} Another popular attack goal is to degrade the model performance such that it can no longer accomplish certain tasks as usual. For example, ~\cite{maus2023adversarialprompting}, a direct and black-box attack, is able to find phrases that effectively bias image-generating LLMs to produce unexpected images when prepended to benign prompts;~\cite{shu2023exploitability}, an indirect and data-poisoning attack, shows that by poisoning the training data used in the fine-tuning process, they can manipulate future models progressed on always claim inability to respond to certain prompts or always include some predefined keywords \eg James in the response.
\end{enumerate}


% To help readers understand the landscape of existing attacks and the positioning of our attack, we summarize the categorization of these attacks in \tabref{tab:attack_summary} (left 4 columns). Note this is not an exhaust list of prior works.

% However, the image generated still looks quite suspicious to humans and the attack only works for a specific single instruction such as "Describe this image". The attack is also fairly easy to be spotted since the sentence the LLM output to tweak its future behavior is explicitly abnormal. 
% We define this as ``prompt injection''. Existing work usually calls this ``Indirect Prompt Injection'', as opposed to ``Prompt Injection'' attacks where the user is intentionally providing malicious prompts to cause the model to behave. We believe this terminology to be confusing and misleading considering that when the user is malicious, it's not precise to call it an injection. Instead, we suggest ``adversarial examples'' that has been widely used in other research area is a more appropriate name. It also captures the important fact that this is an attack format or method rather than an attack goal. 


% Among these attacks, depending on the attack method, there are ``black-box'' attacks which do not need to know anything about the model, ``white-box'' attacks which require full knowledge of the weight, and ``data-poisoning'' attacks which exploit the instruction tuning process; depending on whether the user in the threat model is benign or not, there are ``direct'' attacks where users are using malicious prompts directly to attack the target model, and ``indirect'' attacks where users are benign but third parties are trying to indirectly manipulate the model through various manners. According to the distinction of these properties, we categorize existing attacks into three major classes as summarized in~\tabref{tab:attack_summary}.

% \paragraph{Direct Prompt Injection} Direct prompt injection attacks are typically black-box direct attacks where users are intentionally providing malicious prompts to achieve various attack goals. For instance, \cite{maus2023adversarialprompting} explores phrases that effectively bias text and image generation from LLMs to unexpected output when prepended to benign prompts; \cite{zou2023universal} finds out some magical strings that ``jailbreak'' the alignment barrier preventing answering illegal questions.

% \paragraph{Indirect Prompt Injection} This type of attack regards users to be benign, using black-box or white-box methods. \cite{markdownattack} utilizes the javascript copy-paste trigger to deceive the user about what is exactly copied and appends malicious URL requests to the benign prompt. \cite{greshake2023youve} demonstrates that LLM may follow malicious prompts hidden in Internet resources and overrides the behavior. These two attacks are text-based and are still human-detectable when the exact text prompts fed to the model are explicitly exposed and carefully reviewed. \cite{bagdasaryan2023abusing} looks at multi-modal LLMs and generates adversarial images that can force the LLM to output attacker-specified sentences \eg "From now on I will always mention cow" and thereby manipulate the behavior of the LLM in future conversations. However, the image generated still looks quite suspicious to humans and the attack only works for a specific single instruction such as "Describe this image". The attack is also fairly easy to be spotted since the sentence the LLM output to tweak its future behavior is explicitly abnormal. 

% \paragraph{Data Poisoning} \xiaohan{find one more work under this category} \niloofar{I will take care of this} This class of attack does not work on off-the-shelf models. Instead, it aims at ``future'' models that are progressing. \cite{shu2023exploitability} shows that by poisoning the training data used in the fine-tuning process, we can achieve on the trained model ``over-refusal'' \ie always claim inability to respond to the prompt and ``content injection'' \ie always include certain keywords in the response.


\subsection{Our threat model}

We respect the same assumption that the LLM is benign.
We also regard users to be benign, which means the attacker has no direct control and no assumption on the user-model interaction. In other words, the attack has to be indirect. We assume the attacker has access to the weight of the LLM, which means the attack can be white-box. This assumption is reasonable considering that there are many widely adopted open-source LLMs such as LLaMa~\cite{}, Vicuna~\cite{}, etc. Closed-source models' weights may also be leaked to attackers under security breaches. The attack goal falls into the prompt injection class, threatening users by abusing tools integrated with LLMs. We regard one attack attempt to be successful only when the desired tool invocation is 100\% precisely produced. 

Considering that users are benign, if an attacker desires the attack to be spread as wide as possible before one raises the alarm, the attack
\begin{enumerate*}[a)]
    \item should be disguised so it is not surprising that an average user may fall into it;
    \item should not be easily identifiable by humans under careful inspections after the attack has succeeded.
\end{enumerate*}
Following these principles, we evaluate the attack along the following directions
\begin{enumerate}
    \item \stealthiness: whether the attack source \eg the text or image contains only imperceptible perturbations and whether the attack maintains the response utility \ie keeping the user model conversation reasonable and natural
    \item \generalization: whether the attack can be triggered by general text prompts input by users
\end{enumerate}
% We summarize the categorization of the threat models of existing attacks and ours in \tabref{tab:attack_summary}. Note that the realisticness properties apply only to indirect attacks (\cite{shu2023exploitability} is an exception because of its unique attack channel and prerequisite).  
% The goal of our attack is to invoke API or function calls unintended by the user through malicious images crafted by us, \textit{stealthily}. The API call initiated could be arbitrarily harmful --- it could delete the entire calendar of this user (if the email tool is available) or send conversation history to us through an API endpoint owned by attackers. We assume the malicious images would be fed to the LLM by the user unintentionally. This is realistic since users may be lured into testing these images that attackers posted on social media or the LLM might accidentally ingests these images while browsing the Internet.


\paragraph{Comparison to Prior Works} Comparing our threat model with different attack goals, our attack goal prompt injection is intrinsic to the alignment barriers on the models and is more concerning to benign end users, especially with numerous 3rd party extensions integrated into the models. 
% (We acknowledge the intellectual merit and commercialization significance of those attack goals.) 
% Since the end users are not benign in these threat models, requirements on realisticness do not apply.
Comparing our proposed threat model with prior works that also have prompt injection as the attack goal such as \cite{markdownattack} and \cite{greshake2023youve}, we enforce a stricter requirement on the stealthiness in our threat model --- their attack can still be relatively easily spotted when the exact text prompts fed to the model are carefully reviewed. But they do not require a white-box model. The threat model of \cite{bagdasaryan2023abusing}, falls short of the requirements on stealthiness and generalization --- their adversarial image looks suspicious to human eyes and can only be triggered by one specific instruction, and the attack breaks the response utility. 
% Refer to the right three columns of \tabref{tab:attack_summary} for a summary.

% We describe the salient info of our attack along with the prior works in~\tabref{tab:attack_summary}. Compared to those direct attacks where users are adversarial, our attack presents a more immediate security threat since benign users will be the potential victim in our settings. Also, making API calls are legit behavior of LLMs compared to the other attacks aiming at jailbreaking, performance degradation, and others. This makes our attack intrinsic and harder to be defended by alignment or other techniques. Compared to \cite{bagdasaryan2023abusing} which shares a relevant threat model to ours, our attack does not presume any conversation that the user will have with the model and should work with a general conversation context; we also require the attack to be stealthy --- there should be no obvious indication that the LLM has been ``hijacked''.

% Compared to prior works of indirect prompt injection, our attack is more generalized and stealthier. Imagining that a user is lured into pasting an interesting image shared by unknown people online as input to the LLM or the LLM by chance takes in this image while browsing the web per user request, we can successfully inject desired instructions and manipulate the behavior of this LLM \eg always send the prior conversation to an API endpoint specified by us. Such an image is benign-looking and works for general conversations rather than being restricted to some fixed text as in prior work. 

==> 0_contents/_dep_40_evaluation.tex <==
\section{Evaluation} \label{sec:eval}
To evaluate the attack, we need to measure how well it generates tool invocation syntax according to the attacker's intentions (success rate for different attack variants), the stealthiness of the attack (both image stealthiness and response utility), and the generalization of the attack to unseen prompts.

% \subsection{Setup}
\xiaohan{@zihan update the rest three paragraphs}
We test the attack on an open-sourced multimodal LLM --- LLaMA Adapter~\cite{zhang2023llama}. In brief, LLaMA Adapter encodes an image into a sequence of representations, which are treated as tokens and appended to the text input, such that token generation would be conditioned on the image. From now on, we refer to LLaMA Adapter as the \textit{model}. Note that our attacks are only applied to the image part of the input prompt. 
% With a slight abuse of notation, we will also refer to LLaMA Adapter with a clean, natural image as a clean model, and LLaMA Adapter with our adversarially perturbed image as the attacked model.

For our attack method, we set $\alpha = 0.01, \lambda_i = 0.02, \lambda_r = 1.0$ and train for 12000 steps with a batch size of 1. Details on how the numbers are picked are in Appendix~\ref{app:train}. We observed significant randomness during adversarial image training. In some cases, different trials (where the only difference is the random seed) can lead to an almost perfect attack and a completely failed attack. Therefore, for all experiments, \revise{we report the best result among three trials since attackers can test the performance themselves and always present the best-performing image in public to lure users to use.}

Attackers will choose the best-performing image to work with in practice. Nevertheless, to demonstrate that our method works generically regardless of the base image choice, we sample six images with distinct characteristics and sources in our evaluation. The first two images are AI-generated. One is the logo of LLaMA Adapter and the other one is created by stable diffusion
\footnote{\url{https://stablediffusionweb.com/\#demo}} 
with the prompt ``Create me a beautiful image''. The rest four images are randomly sampled from Shutterstock (free version). These images are photos taken in the real world by various photographers with various subjects. Due to space limitation, we present these images and the preprocessing/sampling details in Appendix~\ref{app:image}. 

\begin{figure*}[t]
    \centering
    % \includegraphics[width=\textwidth]{2_images/attack_success.pdf}
    \begin{adjustbox}{width=0.9\linewidth}
        \input{3_tikz/attack_success}
    \end{adjustbox}
    \caption{Illustration of various cases of attacks. Note that the texts marked in green, same as in~\figref{fig:demo}, are tool invocations that will not be printed out and are invisible to users. Texts marked in red are errors of the invocation syntax.
    % The successful case is shown as a reference.  %\zihan{sorry for another request to update --- do you think it would be better if we highlight the response part and the tool usage part in the image?}
    % b) presents the case with exact score 0 and syntax score 1. c) presents the case with exact score 0 and syntax score 0, where the user will see the weird text in the end and d) shows the case where no invocation attempt is made (exact=0, syntax=0). 
    }
    \label{fig:attack_success}
\end{figure*}


\subsection{Dataset Construction}
\label{Sec: dataset}
To evaluate the generalizability of our attack, we create prompt datasets for training and evaluation independently under two categories: (1) prompts that are related to images (image-related) and (2) prompts that are unrelated to images (image-unrelated). 

For training, the image-related prompts are obtained by querying GPT-4 with the prompt: ``Generate 100 questions related to an image''. These questions are applicable to any general image, but the responses should be varied and specific to each image. The image-unrelated prompts are the first 3200 questions in the Alpaca instruction following dataset~\cite{alpaca}.

For testing, we consider an in-domain generalization setup where the image-related prompts are created by a human volunteer instructed to create 50 different prompts similar to the prompts in the training set and the image-unrelated prompts are a disjoint set of 100 questions in the Alpaca dataset.
Additionally, to better evaluate the generalization of our attack, we create an out-domain test set. As for the image-related prompts, we first generate a textual summary of the image through Bard, and then prompt GPT-4 with the summary and ask it to generate 50 questions given the image summary. Note that the questions for each image would be different in this case. For the image-unrelated prompts, we prompt GPT-4 to generate 50 general questions.

Note that for the instructions from the Alpaca dataset, we omit prompts that contain an input section, and prompts that are too long, to keep most generations under a reasonable length of 128 tokens to speed up training. This leaves us 1803 out of 3200 image-related prompts for training, and 64 out of 100 image-unrelated prompts for evaluation. Since the training set size of unrelated prompts is much larger than the related prompts, during training, we mix them with a ratio of $85:15$.

\subsection{Metrics}
\begin{table*}[t]
\small
    \centering
    \caption{Evaluation of our attack with base image 1 on image stealthiness (SSIM,  L$_2$ and  L$_{\textrm{inf}}$), attack success rate (Syntax/Exact \%), and response utility (Loss) on the in-domain test set for image-related and -unrelated prompts.}
    \resizebox{\linewidth}{!}{
    \renewcommand{\arraystretch}{1.2}
    \input{1_tables/baseimg1_result}
    }
    \label{tab:main_exps}
    \vspace{0.4\baselineskip}
% \vspace{0.5em}
%     \caption{Evaluation of the trained attack from~\tabref{tab:main_exps} on out-domain test set. We pick only the three easier attack types as they are mostly successful in the in-domain setting.}    
%     \resizebox{\linewidth}{!}{
%     \input{1_tables/outdomain_exp}
%     \label{tab:outdomain_exps}
%     }
\end{table*}


We feed our adversarial images to the model against prompts in the test datasets and obtain one response for each prompt. To evaluate the success and stealthiness of our attack, we consider three measures: the fraction of cases where the model emits a tool usage instruction in the response according to the attacker's intent (success rate), the similarity between the perturbed image and the clean image (image stealthiness), and the indistinguishability between the model responses with and without the attack present in terms of being reasonable and natural (response utility). 
\smallskip

\noindent\textbf{Attack Success.}
A successful attack would require an exact reproduction of the tool invocation instruction (exact match). However, a tool invocation may be produced with correct syntax but wrong arguments and fail (syntax match). We measure and report the \textit{proportion} of these two cases among all tested prompt-response pairs as following two metrics (find examples in~\figref{fig:attack_success}).
% Attack success rate is measured by the probability of a precise tool invocation, which we divide into two sub-metrics: the syntax matching score and the exact matching score. In~\figref{fig:attack_success} we show an illustration of these two metrics.
 
\begin{itemize}[nosep=*,leftmargin=*]
    \item \textbf{Syntax.} Syntax match checks whether the tool invocation instruction in the generated response follows the correct syntax. The syntax here refers to a sequence of characters that is specific to each tool. For example, in \deleteemail attack the correct syntax consists of the tool name \texttt{delete\_email} and a string argument \texttt{which=""}, wrapped by a pair of brackets. When the syntax is matched, the LLM will execute the tool with the arguments provided --- whether the execution is exactly following the attacker's intention depends on whether the arguments are precise. Failed syntax matches \eg wrong or partial function/argument keywords, will not be parsed by the LLM, and those texts will be printed out and be seen by users.
    \item \textbf{Exact.} Exact match measures whether the generated instruction in the response is exactly the same as the desired tool invocation. Note that an exact match is \textit{always} a syntax match.
    
\end{itemize}



\smallskip

\noindent\textbf{Image Stealthiness.}
We measure the visual difference between the perturbed adversarial image and its original. The more similar the two images are, the better the stealthiness of the attack. We use the popular Structural Similarity Index Measure (SSIM) for quantification. An SSIM score of $\geq0.9$ is typically not distinguishable to humans: an example is shown in Appendix~\ref{app:ssim}. We also look at the L$_2$ and L$_\infty$ norm of the difference between the adversarial and clean base image as a reference.

\smallskip

\noindent\textbf{Response Utility.}
Response utility is best measured by humans' opinions on whether the conversation between the user and model looks reasonable and natural.  However, since full coverage of human annotations is impossible in large-scale experiments \eg our in- and out-domain test sets, we need a reliable automated metric that best represents the human preference scores. 

In seek of it, we first conduct a small-scale human study on a subset of the test set. We collect two generated responses per question, one with the attack present (with an adversarial image) and one without the attack (with a clean image) for all 214 questions in the in-domain test set.\footnote{50 image-related questions for 3 images and 64 image-unrelated questions.} We ask human annotators to judge whether a response is natural and reasonable with respect to the question as well as the image. Each prompt-response pair is judged by three graduate students majoring in Computer Science unrelated to this project and we obtain the final result with a majority vote to get rid of unusual preferences. 

Then we select the best metric out of four automated metrics: Training Cross Entropy \textit{Loss}, GPT-4 \textit{Selection}, \textit{BLEU} score and \textit{Rouge} scores. To guide the decision, we compare 1) the relative value changes of these metrics with adversarial versus clean image to the value changes of human preference, and 2) the AUC ROC score of each of them computed against the human preference scores. We find that the \textit{Loss} metric correlates with the human preference the best in both cases. Details can be found in~\apref{app:human_eval}. We therefore decide to use \textit{Loss} as the metric of response utility in the evaluation.

Yet, another possible concern is whether the averaged response utility metric would be misleading --- is it possible that the responses are less likely to be reasonable when the adversarial image successfully triggers a correct tool invocation? We verified that this is not the case in~\apref{app:attack_success_utility}.

%\footnote{We tried to use other multimodal LLMs to imitate the human annotation but failed with poor results. Commercial ones like Bard are better but have not yet granted us API access. Leave as future work.}

\subsection{Experiment Results}



\noindent\textbf{The attack is successful, stealthy, and generalizable.} In~\tabref{tab:main_exps} we list the evaluation results of our attack method with base image 1 on the in-domain test set. The corresponding adversarial images generated are listed in~\figref{fig:baseimg1_result}. For the first two attack goals \deleteemail and \sendemail, the success rate are close to 100\% on the image-related set and around 80\% on the image-unrelated set. For all attack variants, the SSIM score is close to 100\%, and the Loss metric shows around 10\% less preference than clean model generations, aligned with the results in~\tabref{tab:reasonable_context}. Even though the success rates for the latter two more challenging attacks are relatively lower, it is fine because as long as the attack remains stealthy, it will take effect and harm users after spreading to enough victims. Due to space limiation, we put the results on other base images in~\apref{}. A similar pattern across these other images are also observed, which shows that our attack works generically with various base images.

% \noindent\textbf{The attack is also generalizable to out-domain samples.} In~\tabref{tab:outdomain_exps} we evaluate on the unseen, out-domain samples from the out-domain test set, using the same adversarial images in~\tabref{tab:main_exps}. The results indicate that the attacked images transfer almost equally well to out-domain examples.

% We also experiment on the ability of generalizing adversarial images to out-domain test samples. The results in Appendix~\ref{app:}indicate that the attacked images transfer almost equally well to out-domain examples
\noindent\textbf{The attack is customizable in favor of various metric.} We also verified that (1) the response utility controlling variable $\lambda_r$ improves the response utility and (2) we can sacrifice image stealthiness to make the attack more likely to be successful for hard attack variants in~\apref{app:hyper_exps}. These bring more flexibility and customizability to the attack according to different use cases.

\noindent\textbf{Transferability across models is not seen.} Meanwhile, considering that we have two backbone models, it's natural to test whether the adversarial image generated on one model could trigger the tool invocation format on the other model. Unfortunately, we were not able to find this happening. None of the image generated on one model was able to generate a ``syntax match'' with any of the prompts in the test set on the other model. We also tested this on black-box models such as Gemini and GPT4o and it was also not successful.

==> 0_contents/tmp_results.tex <==
(0.05, 1.0)  &  book\_ticket  &  pic2  &  42  &  0.96  &  9.46  &  0  &  0  &  1.09  &  0  &  0  &  0.75\\
(0.05, 1.0)  &  book\_ticket  &  pic2  &  43  &  0.94  &  19.36  &  0  &  0  &  1.13  &  0  &  0  &  0.79\\
(0.05, 1.0)  &  book\_ticket  &  pic2  &  44  &  0.95  &  16.39  &  0  &  0  &  1.18  &  0  &  0  &  0.78\\
(0.05, 1.0)  &  book\_ticket  &  pic3  &  42  &  0.93  &  10.75  &  0  &  0  &  1.16  &  0  &  0  &  0.8\\
(0.05, 1.0)  &  book\_ticket  &  pic3  &  43  &  0.95  &  7.23  &  0  &  0  &  1.15  &  0  &  0  &  0.85\\
(0.05, 1.0)  &  book\_ticket  &  pic3  &  44  &  0.94  &  9.53  &  0  &  0  &  1.02  &  0  &  0  &  0.74\\
(0.05, 1.0)  &  delete\_email  &  pic2  &  42  &  0.94  &  15.26  &  0  &  0  &  1.02  &  0  &  0  &  0.77\\
(0.05, 1.0)  &  delete\_email  &  pic2  &  43  &  0.95  &  13.2  &  82  &  82  &  1.08  &  42  &  42  &  0.77\\
(0.05, 1.0)  &  delete\_email  &  pic2  &  44  &  0.95  &  13.02  &  0  &  0  &  1.1  &  0  &  0  &  0.73\\
(0.05, 1.0)  &  delete\_email  &  pic3  &  42  &  0.94  &  9.6  &  0  &  0  &  0.98  &  0  &  0  &  0.88\\
(0.05, 1.0)  &  delete\_email  &  pic3  &  43  &  0.94  &  9.68  &  98  &  98  &  1.06  &  77  &  77  &  0.78\\
(0.05, 1.0)  &  delete\_email  &  pic3  &  44  &  0.94  &  7.99  &  100  &  100  &  1.13  &  72  &  72  &  1.01\\
(0.05, 1.0)  &  send\_email1  &  pic2  &  42  &  0.95  &  12.77  &  96  &  66  &  1.12  &  36  &  19  &  0.83\\
(0.05, 1.0)  &  send\_email1  &  pic2  &  43  &  0.95  &  16.12  &  90  &  88  &  1.11  &  53  &  50  &  0.79\\
(0.05, 1.0)  &  send\_email1  &  pic2  &  44  &  0.95  &  13.35  &  0  &  0  &  1.11  &  0  &  0  &  0.74\\
(0.05, 1.0)  &  send\_email1  &  pic3  &  42  &  0.95  &  7.36  &  2  &  0  &  1.07  &  2  &  0  &  0.78\\
(0.05, 1.0)  &  send\_email1  &  pic3  &  43  &  0.94  &  7.83  &  98  &  96  &  1.06  &  61  &  52  &  0.77\\
(0.05, 1.0)  &  send\_email1  &  pic3  &  44  &  0.93  &  11.4  &  100  &  100  &  1.1  &  73  &  70  &  0.81\\
(0.0, 0.0)  &  send\_email2  &  pic1  &  42  &  0.8  &  37.77  &  90  &  0  &  3.19  &  75  &  0  &  10.42\\
(0.0, 0.0)  &  send\_email2  &  pic1  &  42  &  0.84  &  25.63  &  94  &  94  &  1.81  &  61  &  41  &  2.83\\
(0.0, 0.0)  &  send\_email2  &  pic1  &  42  &  0.84  &  26.3  &  92  &  84  &  1.37  &  59  &  38  &  2.89\\
(0.0, 1.0)  &  send\_email2  &  pic1  &  42  &  0.81  &  34.55  &  94  &  94  &  1.14  &  31  &  27  &  0.82\\
(0.0, 1.0)  &  send\_email2  &  pic1  &  42  &  0.81  &  45.53  &  100  &  100  &  1.05  &  73  &  72  &  0.73\\
(0.0, 1.0)  &  send\_email2  &  pic1  &  42  &  0.84  &  29.17  &  90  &  0  &  1.16  &  44  &  0  &  0.84\\
(0.05, 0.0)  &  send\_email2  &  pic1  &  42  &  0.91  &  12.71  &  100  &  74  &  1.53  &  89  &  66  &  2.28\\
(0.05, 0.0)  &  send\_email2  &  pic1  &  42  &  0.93  &  10.15  &  2  &  2  &  1.39  &  6  &  3  &  0.91\\
(0.05, 0.0)  &  send\_email2  &  pic1  &  42  &  0.93  &  10.4  &  2  &  0  &  1.47  &  5  &  0  &  1.48\\
(0.05, 0.1)  &  send\_email2  &  pic1  &  42  &  0.92  &  11.17  &  100  &  98  &  1.27  &  72  &  64  &  1.04\\
(0.05, 0.1)  &  send\_email2  &  pic1  &  42  &  0.92  &  11.52  &  30  &  30  &  2.05  &  33  &  19  &  3.78\\
(0.05, 0.1)  &  send\_email2  &  pic1  &  42  &  0.93  &  8.71  &  96  &  96  &  1.27  &  50  &  47  &  1.03\\
(0.05, 1.0)  &  send\_email2  &  pic1  &  42  &  0.92  &  11.17  &  16  &  16  &  1.16  &  5  &  5  &  0.87\\
(0.05, 1.0)  &  send\_email2  &  pic1  &  42  &  0.93  &  8.43  &  100  &  98  &  1.21  &  61  &  61  &  0.78\\
(0.1, 0.0)  &  send\_email2  &  pic1  &  42  &  0.93  &  10.73  &  52  &  0  &  1.22  &  25  &  0  &  0.97\\
(0.1, 0.0)  &  send\_email2  &  pic1  &  42  &  0.93  &  11.76  &  0  &  0  &  1.45  &  0  &  0  &  1.26\\
(0.1, 0.0)  &  send\_email2  &  pic1  &  42  &  0.95  &  6.45  &  68  &  38  &  2.32  &  28  &  2  &  3.17\\
(0.1, 0.1)  &  send\_email2  &  pic1  &  42  &  0.95  &  5.78  &  40  &  0  &  1.68  &  16  &  0  &  1.61\\
(0.1, 0.1)  &  send\_email2  &  pic1  &  42  &  0.95  &  6.98  &  0  &  0  &  1.21  &  0  &  0  &  0.9\\
(0.1, 1.0)  &  send\_email2  &  pic1  &  42  &  0.95  &  5.89  &  8  &  6  &  1.09  &  8  &  6  &  0.8\\
(0.1, 1.0)  &  send\_email2  &  pic1  &  42  &  0.95  &  6.27  &  94  &  94  &  1.12  &  45  &  45  &  0.84\\
(0.1, 1.0)  &  send\_email2  &  pic1  &  42  &  0.95  &  6.97  &  0  &  0  &  1.07  &  0  &  0  &  0.78\\
    \hline
    \hline
(0.02, 1.0)  &  book\_ticket  &  pic1  &  42  &  0.88  &  18.33  &  0  &  0  &  1.17  &  0  &  0  &  0.95\\
(0.02, 1.0)  &  book\_ticket  &  pic1  &  43  &  0.9  &  15.8  &  22  &  20  &  1.51  &  9  &  8  &  0.97\\
(0.02, 1.0)  &  book\_ticket  &  pic1  &  44  &  0.88  &  20.1  &  0  &  0  &  1.19  &  0  &  0  &  0.82\\
(0.02, 1.0)  &  book\_ticket  &  pic2  &  42  &  0.94  &  16.87  &  0  &  0  &  1.23  &  0  &  0  &  0.82\\
(0.02, 1.0)  &  book\_ticket  &  pic2  &  43  &  0.94  &  14.77  &  0  &  0  &  1.19  &  0  &  0  &  0.74\\
(0.02, 1.0)  &  book\_ticket  &  pic2  &  44  &  0.93  &  31.23  &  0  &  0  &  1.14  &  0  &  0  &  0.76\\
(0.02, 1.0)  &  book\_ticket  &  pic3  &  42  &  0.91  &  14.51  &  0  &  0  &  1.04  &  0  &  0  &  0.85\\
(0.02, 1.0)  &  book\_ticket  &  pic3  &  43  &  0.91  &  15.42  &  46  &  44  &  1.3  &  9  &  9  &  1.07\\
(0.02, 1.0)  &  book\_ticket  &  pic3  &  44  &  0.9  &  17.19  &  0  &  0  &  1.04  &  0  &  0  &  0.73\\
(0.02, 1.0)  &  delete\_email  &  pic1  &  42  &  0.91  &  11.52  &  98  &  98  &  1.09  &  78  &  78  &  0.8\\
(0.02, 1.0)  &  delete\_email  &  pic1  &  43  &  0.89  &  15.19  &  0  &  0  &  1.09  &  0  &  0  &  0.74\\
(0.02, 1.0)  &  delete\_email  &  pic1  &  44  &  0.91  &  11.7  &  100  &  100  &  1.09  &  58  &  58  &  0.79\\
(0.02, 1.0)  &  delete\_email  &  pic2  &  42  &  0.92  &  29.78  &  90  &  90  &  1.11  &  55  &  55  &  0.82\\
(0.02, 1.0)  &  delete\_email  &  pic2  &  43  &  0.93  &  17.66  &  34  &  34  &  1.18  &  28  &  28  &  0.89\\
(0.02, 1.0)  &  delete\_email  &  pic2  &  44  &  0.94  &  17.99  &  60  &  60  &  1.14  &  25  &  25  &  0.77\\
(0.02, 1.0)  &  delete\_email  &  pic3  &  42  &  0.9  &  15.21  &  98  &  98  &  1.07  &  50  &  50  &  0.84\\
(0.02, 1.0)  &  delete\_email  &  pic3  &  43  &  0.87  &  24.45  &  92  &  92  &  1.11  &  73  &  73  &  0.78\\
(0.02, 1.0)  &  delete\_email  &  pic3  &  44  &  0.88  &  22.03  &  80  &  80  &  1.08  &  56  &  56  &  0.79\\
(0.02, 1.0)  &  send\_email1  &  pic1  &  42  &  0.9  &  15.56  &  98  &  98  &  1.08  &  69  &  69  &  0.77\\
(0.02, 1.0)  &  send\_email1  &  pic1  &  43  &  0.89  &  16.03  &  100  &  100  &  1.14  &  67  &  61  &  0.87\\
(0.02, 1.0)  &  send\_email1  &  pic1  &  44  &  0.88  &  17.7  &  98  &  96  &  1.18  &  55  &  52  &  0.76\\
(0.02, 1.0)  &  send\_email1  &  pic2  &  42  &  0.93  &  18.32  &  22  &  0  &  1.08  &  23  &  0  &  0.8\\
(0.02, 1.0)  &  send\_email1  &  pic2  &  43  &  0.93  &  17.42  &  92  &  92  &  1.18  &  61  &  58  &  0.88\\
(0.02, 1.0)  &  send\_email1  &  pic2  &  44  &  0.92  &  22.53  &  8  &  4  &  1.85  &  6  &  2  &  0.91\\
(0.02, 1.0)  &  send\_email1  &  pic3  &  42  &  0.91  &  14.72  &  90  &  90  &  1.02  &  70  &  67  &  0.8\\
(0.02, 1.0)  &  send\_email1  &  pic3  &  43  &  0.87  &  22.15  &  0  &  0  &  1.09  &  0  &  0  &  0.77\\
(0.02, 1.0)  &  send\_email1  &  pic3  &  44  &  0.92  &  12.61  &  100  &  100  &  1.04  &  69  &  69  &  0.78\\
(0.02, 1.0)  &  send\_email2  &  pic1  &  42  &  0.85  &  24.18  &  84  &  82  &  1.27  &  42  &  41  &  0.91\\
(0.02, 1.0)  &  send\_email2  &  pic1  &  43  &  0.86  &  21.9  &  76  &  74  &  1.17  &  34  &  28  &  0.81\\
(0.02, 1.0)  &  send\_email2  &  pic1  &  44  &  0.91  &  11.6  &  100  &  100  &  1.14  &  61  &  56  &  0.86\\
(0.02, 1.0)  &  send\_email2  &  pic2  &  42  &  0.92  &  22.98  &  0  &  0  &  1.16  &  0  &  0  &  0.78\\
(0.02, 1.0)  &  send\_email2  &  pic2  &  43  &  0.91  &  27.37  &  100  &  68  &  1.08  &  48  &  31  &  0.87\\
(0.02, 1.0)  &  send\_email2  &  pic2  &  44  &  0.91  &  25.88  &  0  &  0  &  1.66  &  2  &  0  &  1.01\\
(0.02, 1.0)  &  send\_email2  &  pic3  &  42  &  0.87  &  25.12  &  52  &  0  &  1.24  &  13  &  0  &  0.95\\
(0.02, 1.0)  &  send\_email2  &  pic3  &  43  &  0.88  &  19.85  &  86  &  0  &  1.19  &  31  &  0  &  0.78\\
(0.02, 1.0)  &  send\_email2  &  pic3  &  44  &  0.89  &  20.73  &  0  &  0  &  1.19  &  5  &  0  &  0.9\\

==> 3_tikz/standalone.tex <==
%
%\iffalse
%<*tex>
% \fi
% \subsection{Simple TeX File}
%
%    \begin{macrocode}
%%\ProvidesFile{standalone.tex}[2010/02/28 v0.4 Provides if-switch to show if file is compiled standalone]%
%    \end{macrocode}
%
% \begin{macro}{\ifstandalone}
% Provides \cs{ifstandalone} switch which is |\iftrue| if the normal |\documentclass|
% was not yet executed (and subsequently redefined to be |\@twoclasseserror|).
%    \begin{macrocode}
\expandafter\ifx\csname ifstandalone\endcsname\relax
\expandafter\newif\csname ifstandalone\endcsname
\expandafter\ifx\csname @twoclasseserror\endcsname\documentclass
\else
  \standalonetrue
\fi
\fi
%    \end{macrocode}
% \end{macro}
%
% \iffalse
%</tex>
% \fi
%
